Not So Fast: Analyzing the Performance of WebAssembly vs. Native Code

All major web browsers now support WebAssembly, a low-level bytecode intended to serve as a compilation target for code written in languages like C and C++. A key goal of WebAssembly is performance parity with native code; previous work reports near parity, with many applications compiled to WebAssembly running on average 10% slower than native code. However, this evaluation was limited to a suite of scientific kernels, each consisting of roughly 100 lines of code. Running more substantial applications was not possible because compiling code to WebAssembly is only part of the puzzle: standard Unix APIs are not available in the web browser environment. To address this challenge, we build Browsix-Wasm, a significant extension to Browsix that, for the first time, makes it possible to run unmodified WebAssembly-compiled Unix applications directly inside the browser. We then use Browsix-Wasm to conduct the first large-scale evaluation of the performance of WebAssembly vs. native. Across the SPEC CPU suite of benchmarks, we find a substantial performance gap: applications compiled to WebAssembly run slower by an average of 45% (Firefox) to 55% (Chrome), with peak slowdowns of 2.08x (Firefox) and 2.5x (Chrome). We identify the causes of this performance degradation, some of which are due to missing optimizations and code generation issues, while others are inherent to the WebAssembly platform.

==> background.tex <==
\section{Background}

This section introduces \wasm and its predecessor, \asmjs.

\subsection{\asmjs}

\asmjs is a subset of JavaScript introduced in 2013 that is statically typed and can be efficiently compiled~\cite{asmjs:nightly,asmjs}.
\asmjs exposes a computation model that closely matches what C and C++ programs are designed for, with fast loads and stores to linear memory, separate integer and floating point arithmetic, along with functions and function pointers~\cite{asmjs:spec}.
As such, \asmjs is designed as a compilation target rather than a language developers are expected to write by hand.

\asmjs showed that large, complex software like the Unreal 3 3D video game engine could run in the browser with near-native performance (less than a 2$\times$ slowdown)~\cite{unreal,asmjs:announcement}.

As \asmjs is strictly a subset of JavaScript, it is limited by all of the constraints of JavaScript.
JavaScript has significant parsing overhead -- the same program compiled to WebAssembly can be parsed an order of magnitude faster than \asmjs~\cite{wasm-faster-asmjs}.
Additionally, JavaScript doesn't support 64-bit integers, so while 64-bit integer types and operations may be available natively, they must be emulated in \asmjs.

\subsection{\wasm}

\wasm{} is a typed low-level bytecode, defined as a programming language with formal semantics~\cite{webassembly, haas:2017:webassembly}.
These semantics are hardware independent, and ensure that valid bytecode (bytecode that typechecks) is safe to execute and easy to reason about.
Integers (both 32-bit and 64-bit) are distinct from floating point numbers (in a change from JavaScript), and operator bytecodes are specific to the operand types.
Additionally, \wasm only supports structured control flow, rather than arbitrary branches and gotos.
Structured control flow means that branches can only target in-scope labels.
This ensures that code can be validated for correctness in a single pass.

\wasm programs have access to a large array of bytes referred to as linear memory.
This linear memory is disjoint from the execution stack, program bytecode and JIT code, and the browser engine's internal data structures.
This strict separation ensures that buggy or malicious \wasm{} programs can only corrupt their own computations, not compromise the memory safety of JavaScript running in the same context or browser security.

Indirect function calls are one of the most significant departures from
native code. With indirect function calls, control flow passes through 
a table of function pointers which is present in each \wasm{} module.
The selected function pointer is type-checked at runtime to ensure
type and memory safety, no such checks are done in native C and 
C++ binaries.

%TODO: Add a Hello World example

%~ A \wasm module has to be instantiated before
%~ it can be executed by the embedder, like JavaScript VM. Each function 
%~ takes \wasm values as parameters and retunrs a sequence of 
%~ results. Each function executes a sequence of instructions, which are 
%~ based on a stack machine. Each instruction pops values from the implicit 
%~ operand stack and push resulting values on it. Due to the type system, 
%~ the layout of operand stack can be statically determined at any point 
%~ in the code. A function can contains local variables and modify global 
%~ variables. WebAssembly support integers and IEEE 754 floating point 
%~ numbers of 32 and 64 bit width. 


%~ WebAssembly is a web standard that defines a binary format and a assembly
%~ like text format for executable code.  Low level code written in WebAssembly can 
%~ be compiled to native code ahead-of-time, thereby, providing near native
%~ performance. Due to its architecture independent byte code and its 
%~ features, applications written in (or compiled to) WebAssembly are 
%~ portable over different machines, operating systems, and browsers. 
%~ Parsing, transmitting, and loading time of web applications code over a 
%~ network can affect the overall responsiveness of applications, 
%~ WebAssembly has a compact binary format representation. Hence, 
%~ WebAssembly solves two key issues: (i) executing native applications on 
%~ browsers with near native speed, memory safety, and portability, (ii) 
%~ providing a compact representation to improve the responsiveness of 
%~ applications.

%~ Each binary in WebAssembly takes the form of a {\it module}, which
%~ contains definitions for \textit{functions}, {\it global} variables, 
%~ {\it tables}, and {\it memories}. Each definition can be exported or 
%~ imported by modules.
%~ A WebAssembly module has to be instantiated before
%~ it can be executed by the embedder, like JavaScript VM. Each function 
%~ takes WebAssembly values as parameters and retunrs a sequence of 
%~ results. Each function executes a sequence of instructions, which are 
%~ based on a stack machine. Each instruction pops values from the implicit 
%~ operand stack and push resulting values on it. Due to the type system, 
%~ the layout of operand stack can be statically determined at any point 
%~ in the code. A function can contains local variables and modify global 
%~ variables. WebAssembly support integers and IEEE 754 floating point 
%~ numbers of 32 and 64 bit width. 

%~ A WebAssembly program has a large array of bytes referred to as a
%~ {\it linear memory} as its memory. The unit of the size of memory is a 
%~ page, which is defined to be 64 KiB. The effective memory address of is 
%~ a 32-bit integer, hence, the module can access a maximum of 4GB of 
%~ memory. Linear memory is disjoint from code space, the execution stack, 
%~ and the engine's data structures; therefore compiled programs cannot 
%~ corrupt their execution environment, jump to arbitrary locations, or 
%~ perform other undefined behavior. 


==> charts.tex <==
% AUTOGENERATED by ./r/gen -- DO NOT EDIT


==> future_directions.tex <==
\section{Future Directions}
Better Code Generator: Register Allocator, Instruction Selection,
Removing unnecessary branch statements


%~ \section{Events meaning}
%~ Source: \url{http://web.eece.maine.edu/~vweaver/projects/perf_events/perf_event_open.html}

%~ \begin{itemize}
    %~ \item{instructions: retired instructions}
    %~ \item{cache-references: last level cache accesses}
    %~ \item{cache-misses: last level cache misses}
    %~ \item{branch-instructions: retired branch instructions. same as branch-instructions-retired}
    %~ \item{branch-misses: mispredicted branch instructions.}
    %~ \item{L1-dcache-load-misses:}
    %~ \item{L1-dcache-loads:}
    %~ \item{L1-dcache-stores:}
    %~ \item{L1-icache-load-misses:}
    %~ \item{LLC-load-misses:}
    %~ \item{LLC-loads:}
    %~ \item{LLC-stores:}
    %~ \item{branch-load-misses: branch load misses from branch prediction unit}
    %~ \item{branch-loads: branch loads from branch prediction unit}
    %~ \item{dTLB-load-misses: }
    %~ \item{dTLB-loads:}
    %~ \item{iTLB-load-misses:}
    %~ \item{iTLB-loads:}
    %~ \item{branch-instructions-retired: Same as branch-instructions.}
    %~ \item{branch-misprediction-retired: same as branch-misses}
    %~ \item{all-branch-mispredictions:}
    %~ \item{conditional-branch-mispredictions:}
    %~ \item{all-branches: same as branch-instructions above.}
    %~ \item{conditional-branches:}
    %~ \item{near-returns:}
    %~ \item{L1-load-hit:}
    %~ \item{L2-load-hit:}
    %~ \item{L3-load-hit:}
    %~ \item{L1-load-miss:}
    %~ \item{L2-load-miss:}
    %~ \item{L3-load-miss:}
    %~ \item{all-loads-retired:}
    %~ \item{all-stores-retired:}
    %~ \item{LLC-misses:}
    %~ \item{LLC-references:}
    %~ \item{instructions-retired: same as instructions above}
    
%~ \end{itemize}

